Data Player: Automatic Generation of Data Videos with Narration-Animation Interplay

Data visualizations and narratives are often integrated to convey data stories effectively. Among various data storytelling formats, data videos have been garnering increasing attention. These videos provide an intuitive interpretation of data charts while vividly articulating the underlying data insights. However, the production of data videos demands a diverse set of professional skills and considerable manual labor, including understanding narratives, linking visual elements with narration segments, designing and crafting animations, recording audio narrations, and synchronizing audio with visual animations. To simplify this process, our paper introduces a novel method, referred to as Data Player, capable of automatically generating dynamic data videos with narration-animation interplay. This approach lowers the technical barriers associated with creating data videos rich in narration. To enable narration-animation interplay, Data Player constructs references between visualizations and text input. Specifically, it first extracts data into tables from the visualizations. Subsequently, it utilizes large language models to form semantic connections between text and visuals. Finally, Data Player encodes animation design knowledge as computational low-level constraints, allowing for the recommendation of suitable animation presets that align with the audio narration produced by text-to-speech technologies. We assessed Data Player's efficacy through an example gallery, a user study, and expert interviews. The evaluation results demonstrated that Data Player can generate high-quality data videos that are comparable to human-composed ones.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/overview.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.7\linewidth]{figures/pipeline.png}
\caption{The pipeline of automatic generation of narration-animation interplay for data videos} 
\label{fig: pipeline}
\end{figure*}

\section{Design Overview}
The main goal of \tool is to automatically generate narration-animation interplay for data videos, accepting static narration text and static visualization design as input. By eliminating technical barriers and enabling users to focus on the creative aspects of video production, we hope to empower more people to create high-quality data videos to share their insights and research findings. This section discusses the design requirements of the workflow and introduces the automatic creation pipeline.






\iffalse
\subsection{Automatic Creation Workflow}
We need an automatic creation workflow to generate data video alternatives and references to help designers apply our proposed design guidelines. The Z3 \cite{jensen_tools_2006} constraint solver is used to solving the above constraints throughout the workflow.

\subsubsection{Processing Visualization and Text}
Static visualizations and narratives are input in the form of SVG graphics and plain text, respectively. Our approach first establishes the links between visual elements and narrative entities. To be specific, we first identify the visual elements of the visualization inputs that can be animated and extract keywords from them. Then we leveraged the keywords to link visual elements with entities in narration by calculating semantic similarity supported by the BERT model.

\subsubsection{Generating Audio and Animation}
Generating data videos requires the preparation of audio and animation materials. We leverage text-to-speech techniques to generate audio voiceover for the data video. To enable animation timeline generation, a time-aligned script was acquired. The text-to-speech services return the audio file and the timestamp of each word. Commercial services such as Google Text-to-Speech, Microsoft Azure, and Amazon Polly can be alternatively used.

A set of predefined animation actions can be directly applied to the animations. We specify animation effects in four types of animation actions from the library for each visual element based on semantic constraints. Then our approach seeks to automatically organize animation sets in alignment with the generated audio timeline. It makes temporal decisions to allocate using constraint-based programming.

% To generate animations via text description, we need to specify how various animation effects can be used to convey messages from the narration. We categorize the animation effects into four groups developed a set of heuristics to select animation effects from a pre-designed animation library. The animation effect library can enable quickly and flexibly creation of animations in a data video.

\subsubsection{Synthesising Data Video}
We leverage the narration timeline to arrange animation effects applied to the visual elements. The last frame of the previous animation will be retained for the time period when no animation is applied. Moreover, the animations should be coordinated to avoid overwhelming the audience. The animated annotations should also avoid messing up the canvas. We resolved these generic constraints at this stage and synthesise the audio and animation sequences into a data video.
\fi








% ref crosspower
% \copied{Finally, \tool (visualization - text mapping) utilizes BERT to compare embedding between text in visualizations and narrations to enable mapping between the two media. Other algorithms such as xx, and pretrained model and xx are also applicable to solve the problem. The performance of using different techniques can vary across different styles of text and charts and can be chosen alternatively.}
\iffalse
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figures/ui.jpg}
\caption{Narration-Animation Interplay. ''The bar chart illustrates the top 4 economies in the world by GDP.  The USA has the highest GDP at about \$18.5 trillion,  followed by the EU and China at \$15.4 and \$11.8 trillion, respectively.''} \label{timeline}
\end{figure*}


\subsection{User Interface}
In this section, we introduce a user interface to enable designers to intuitively understand and utilize the proposed guidelines. To make the guidelines easy to access, we employed a toggle panel for our automatic approach. Users can intuitively toggle on or off each guideline to see how they will influence the results of generated data videos. Or, they can simply upload their design files, i.e., visualization graphics and narration text, to the interface and get ready-to-use generated videos that satisfy all guidelines. Furthermore, we also provide basic video editing and visual design features.
\fi


